Fast Isogeometric Boundary Element Method based on Independent Field Approximation

An isogeometric boundary element method for problems in elasticity is presented, which is based on an independent approximation for the geometry, traction and displacement field. This enables a flexible choice of refinement strategies, permits an efficient evaluation of geometry related information, a mixed collocation scheme which deals with discontinuous tractions along non-smooth boundaries and a significant reduction of the right hand side of the system of equations for common boundary conditions. All these benefits are achieved without any loss of accuracy compared to conventional isogeometric formulations. The system matrices are approximated by means of hierarchical matrices to reduce the computational complexity for large scale analysis. For the required geometrical bisection of the domain, a strategy for the evaluation of bounding boxes containing the supports of NURBS basis functions is presented. The versatility and accuracy of the proposed methodology is demonstrated by convergence studies showing optimal rates and real world examples in two and three dimensions.

==> results_integration_old.tex <==
\subsection{Single Patch Integration}

The following test investigates the impact of the reduced number of geometry evaluations to the calculation time with respect to the subparametric formulation. Such operations are needed for the calculation of tangents and outward normals to the NURBS patch. The test setting is illustrated in \figref{fig:integration_test_setting}. A linear, flat NURBS patch $\be$ is placed in the $xy$--plane. Three different collocation points are chosen, so that the boundary integral gets singular, nearly singular and regular and thus subject to different integration strategies as described in \secref{sec:integration}. The error of integration is chosen $\err_Q=10^{-9}$. The integration is performed for the discrete single layer $\mat{V}_\be$ and double layer potential $\mat{K}_\be$. For accurate integration, a significant amount of Gauss points are needed. Especially for the singular integration, the amount increases rapidly. This is demonstrated in \tabref{tab:singlePatchIntegration_superparametrix} for this particular case.







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% BENJAMIN SAYS:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Different integrations over a simple unit square, represented by a linear NURBS patch, are performed.
% To study the behaviour of our subparametric approach, we first perform different integrations over a simple unit square.
% This test is used to investigate the influence of the evaluation of geometry related information, particularly the Jacobian, to the simulation time. 




It is placed in the xy--plane and three collocation points are defined.
The first is a corner node of the square which causes singular integration.
The second is very close to the square which yields to nearly singular integration and for the third is far enough away so that a regular integration can be performed.  
The test setting is illustrated in \figref{fig:integration_test_setting}.
% The Poisson's ratio $\nu=0.3$ and a Young's modulus $E=\SI{1.0}{\newton\per\square\meter}$ is assumed.%

%%
\tikzfig{tikz/integration_test_setting}{1.5}
{ 
	Position of the unit square and the collocation points, marked by black dots, for the regular, nearly singular and singular cases.
}{integration_test_setting}
%%
% For each collocation point the single and double layer operator are applied to the patch. 
% The number of required Gauss points, the resulting matrix norm \mycomment[BM]{add definition of norm?} and the integration time are measured.
% The number of Gauss points is determined by the adaptive scheme with the accuracy $\err_Q=10^{-9}$.
% Each integration had been performed 100 times, in order to achieve reliable integration times.

For each collocation point the single and double layer operator are applied to the NURBS patch.
The numerical integration is performed by the adaptive scheme described in \secref{sec:integration}, with an maximum allowed error of $\err_Q=10^{-9}$.
The resulting number of Gauss point for the initial integrand ($p=1$) are listed in  \tabref{tab:singlePatchIntegration_superparametrix}.

\begin{mytable}
{The number of Gauss points used for the numerical integration of the initial and superparametric patch.}
{singlePatchIntegration_superparametrix}
{lcccc}
\mytableheader{ 
	Integration			& Kernel U 			& Kernel T} 
	regular  	& 64					& 64		\\
	nearly singular  	& 375		     	& 415	\\
	singular  	& 1447 			         & 1015 	\\
\end{mytable}

The initial representation is refined by order elevation up to $p=6$.
Thereby, three different patch types are analyzed.
The superparametric case, where only the basis of the geometry is order elevated, the subparametric case, where only the basis of unknowns is order elevated and the isoparametric case, where the basis of both is order elevated.
Note that the integrand change if the basis of unknowns is refined. However, the norm of the resulting vector is only influence by the distance of the collocation point.
% Note that the refinement of superparametric patch does not affect the integrand itself, but the evaluation of the Jacobian. 
% It is also worth noting that all patch type lead to the same results.
% However, the patch type affects the integration time.

% The number of Gauss points for the initial and superparametric patch are shown in \tabref{tab:singlePatchIntegration_superparametrix}.
% In the isoparametric and subparametric case, order elevation modifies the integrand which yields to a variable number of Gauss points.
% They are listed in \tabref{tab:singlePatchIntegration_GP}.
% However, the resulting matrix norm is only influence by the distance of the collocation point.
% They are illustrated in \tabref{tab:singlePatchIntegration_superparametrix}.

For each patch type and order, the numerical integration is performed 100 times and the total integration time is measured.  
In \figref{fig:time_super}, the integration time in the superparametric case $t_{super}$ is related to the integration time of the initial unrefined patch $t_{init}$.
The ratio of the integration time on the conventional isoparametric $t_{iso}$ and the proposed subparametric $t_{sub}$ patch is shown in \figref{fig:time_sub}.\mycomment[BM]{Schrift skaliert mit Bildgröße - groupplot Problem? }


% \begin{mytable}
% {Table with resulting matrix norms and number of Gauss points for the initial and superparametric patch.}
% {singlePatchIntegration_superparametrix}
% {lcccc}
% \mytableheader{ 
% 				& \multicolumn{2}{c}{Kernel U} 			& \multicolumn{2}{c}{Kernel T} \\
% 	\cmidrule(lr){2-3}
% 	\cmidrule(lr){4-5}
% 	Integration 	&  \# Gauss points 	& Matrix norm &  \# Gauss points 	& Matrix norm      }  
% 	regular  	& 64			& 0.414308 		& 64			& 0.0256931 	                     \\
% 	nearly singular  	& 375		& 0.30024        	& 415		& 0.104485   	                     \\
% 	singular  	& 1447 			& 0.315389           & 1015 			& 0.707107  	              \\
% \end{mytable}


% \begin{mytable}
% {Table for number of Gauss points related to the order of the basis for the isoparametric and subparametric patch.}
% {singlePatchIntegration_GP}
% {lcccccc}
% \mytableheader{ 
% 	& \multicolumn{3}{c}{\# GP for Kernel U} & \multicolumn{3}{c}{\# GP for Kernel T} \\
% 	\cmidrule(lr){2-4}
% 	\cmidrule(lr){5-7}
% 	 $p$ 	&  regular &  nearly	&  singular &  regular &  nearly	&  singular  } 
% 	1	&  64	 & 375  &  1447  &  64        &     415    &  1015     \\
% 	2	&  64	 & 375  &  1575  &  100        &    415    &   1015    \\
% 	3	& 100  &375 &  1711    & 100        &    415     &1015      \\
% 	4	& 100  &375 &  1903    & 100        &     479    &1015       \\
% 	5	& 100  &375 &  1967    & 100        &     479    & 1015       \\
% 	6	& 100  &439 &  1967    & 100        &     511    & 1015        \\
% % 	7	& 100  &471 &  2047    & 100        &     575    & 1015        \\
% \end{mytable}

\tikzfig{plots/GP-plane_planestrain_KERNEL_U_and_T_GEOMETRY}{1.0}
{ 
	The integration time of the superparametric patch ($t_{super}$) related to the initial patch ($t_{init}$) for the regular, nearly singular and singular integral with the U kernel (left) and T kernel (right), respectively. 
	The order of the basis functions related to the geometry are denoted by $p$.
% 	The relative integration time for U kernel (left) and T kernel (right). 
% 	Only geometry refinement. Superparametric vs. initial  case.
}{time_super}

% \tikzfig{plots/GP-plane_planestrain_KERNEL_U_and_T_GP}{0.8}
% {
% 	Number of Gauss points if the basis related to the Kernel is order elevated. On the left hand side is the Kernel U and on the right hand side is the Kernel T. 
% }{singlePatchIntegration_GP}

\tikzfig{plots/GP-plane_planestrain_KERNEL_U_and_T_ALL}{1.0}
{
	The integration time of the isoparametric ($t_{iso}$) related to the subparametric ($t_{sub}$) patch for U kernel (left) and T kernel (right).
	The order $p$ corresponds to the refined basis functions.
}{time_sub}

Both time comparisons verify the increasing numerical effort due to the order elevation of the geometry.
It is worth noting that there is hardly any difference between the regular, nearly singular and singular integration, although the number of Gauss points rises rapidly if the collocation point comes closer to the patch.
This indicates that the governing factor of the relative integration time is the efficiency of the geometry evaluation.
The benefit of the subparametric patch is for the Kernel T slightly better because the evaluation of the Kernel includes the outward normal of the surface. 
However, note that accurate integration requires an immense quantity of Gauss points, which leads to a high number of evaluations of geometry related informations.


% In both 
% This indicates the effect of a pure geometry refinement.

% It is apparent that  

% \todos{}
% {
%   \textbf{Text}
% \begin{itemize}
%  \item Do we need the matrix norm and/or the GP information?
%  \item Show only superparametric vs initial?
% \end{itemize}
% 
%   \textbf{Points for discussion}
% \begin{itemize}
% 	\item Accurate integration requires an immense quantity of Gauss points, which leads to a high number of evaluations of geometry related informations.
% 	\item Relative integration time is independent of the number of Gauss points and integration scheme.
% 	The governing factor is the efficiency of the geometry evaluation.
% 	\item The benefit of the subparametric patch is for the Kernel T slightly better because the evaluation of the Kernel includes the outward normal of the surface. 
% \end{itemize}
% }


%% QUAD ERROR %% \paragraph{Circular and Spherical Excavation}
%% QUAD ERROR %% 
%% QUAD ERROR %% To verify the integration routine, we apply a constant hydrostatic load to the boundary of a circular or spherical excavation. The solution space is also circular or spherical and hence, covered by the NURBS functions. The determined point wise error matches the error of integration. The error $\err_Q$ in \eqref{eq:adaptive_integration} has been set differently. Thus, \figref{fig:circular-integration} outlines the accuracy of the adaptive integrator in two dimensions and its invariance to the size of $\mat{V}$ and $\mat{K}$.%
%% QUAD ERROR %% %%
%% QUAD ERROR %% \emptyfig{tikz/circular-integration}{1.0}{Error of integration measured in the maximum norm at points $\tilde{\pt{x}}$ for the discrete single and double layer potential calculated adaptively}{circular-integration}
%% QUAD ERROR %% %%






%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "fastigabem"
%%% eval: (auto-fill-mode -1)
%%% eval: (longlines-mode -1)
%%% ispell-local-dictionary: "en_GB-ise"
%%% End: 

